Look, Read and Ask: Learning to Ask Questions by Reading Text in Images

We present a novel problem of text-based visual question generation or TextVQG in short. Given the recent growing interest of the document image analysis community in combining text understanding with conversational artificial intelligence, e.g., text-based visual question answering, TextVQG becomes an important task. TextVQG aims to generate a natural language question for a given input image and an automatically extracted text also known as OCR token from it such that the OCR token is an answer to the generated question. TextVQG is an essential ability for a conversational agent. However, it is challenging as it requires an in-depth understanding of the scene and the ability to semantically bridge the visual content with the text present in the image. To address TextVQG, we present an OCR consistent visual question generation model that Looks into the visual content, Reads the scene text, and Asks a relevant and meaningful natural language question. We refer to our proposed model as OLRA. We perform an extensive evaluation of OLRA on two public benchmarks and compare them against baselines. Our model OLRA automatically generates questions similar to the public text-based visual question answering datasets that were curated manually. Moreover, we significantly outperform baseline approaches on the performance measures popularly used in text generation literature.

==> rough.tex <==
%A lot of factors in making decisions in everyday tasks depend on interpreting the textual information in this man-made environment. Whether it is checking out the name of the store, or finding the appropriate directions on the sign board which leads you to the destination, understanding and making decisions based on the textual cues in the scene finds its own set of difficulties and needs. The system which can not just recognise the text but essentially which can read and comprehend it, becomes inevitable. 
\newline
%It is common to observe that visually-impared users frequently ask the questions on their devices which largely depend on the text in the image. The existing datasets like ST-VQA which comprises 23,038 images and 31,791 questions and TextVQA dataset which contains 28,408 images and 45,336 questions result as base datasets which provide relationship between the text in the image and the different types of questions that could be asked using the text in the image. Teaching machines the art of asking questions based on the text present in the scene eg, What is the name of the restaurant in the image, What is the title of the book, appeals to be an interesting task to work on.
\newline
%To move towards human-like reasoning, the model should be able to utilize both the visual as well as the textual information in the image. The model must learn to understand the image containing text and formulate an appropriate question with respect to the image and textual information as whole.

%Acknowledging the importance of text, this paper focuses on the task of learning to ask questions by reading the text in the image we propose a simple framework for \prob{} system which constitutes the following representations:


%Image-Token attention vector is obtained using CNN features and text representations which is further concatenated with individual image and token feature vectors along with the positional vector. A multi-modal fusion network combines features from different modalities into c-space which is combined space. This feature vector from combined space is given as the input to the bi-directional LSTM which acts as a question generator. 

%The task of understanding visual cues has been an elemental task in multimodal tasks like Image Captioning, Visual Question Answering (VQA) and Visual Question Generation (VQG). Infact textual cues provide direction towards complete scene understanding. 
%\newline
%Visual Question Answering. Various advancements and new dataset have been introduced since the first work by Antol et al. Goyal et al. addresses the issue of answering without sufficient visual grounding in earlier datasets like DAQUAR or COCO-QA by adding complementary triplets for every original triplet. Existing VQA approaches follow a supervised paradigm that is based on CNN + RNN encoder-decoder formulation[1]. Recently, VQA models also use attention mechanisms to strengthen VQA[all attention based works]. Works such as Wang et al. introduced Fact-Based VQA datasets which explicitly required external knowledge to answer a question.
%\newline
%Visual Question Generation. Generating Natural Questions is a novel task introduced in the work (Generating natural questions about an image) where the system is tasked with asking a natural and engaging question when shown an image. Works in Visual question generation started with algorithmic rule-based [2,3]. Later deep learning approaches like [4,5] were implemented. [7: dual task] presents an end-to-end unified model, which introduces question generation as a dual task of question answering. [6 information maximization] extends visual question generation by treating question generation as a process that maximizes mutual information.
%\newline
%Text detection and recognition is a task which initiates generalisation of VQA system that can integrate textual cues with complete scene understanding.
%Text based image captioning. Based on the content in an image, the image captioning challenges a model to automatically generate a natural language description. Datasets like COCO Captions and Flickr30k, focus on visual objects. TextCaps proposes a dataset which enhances text comprehension in the context of an image. Text captioning requires a model to read and reason about texts and generate coherent descriptions.
%\newline
%Text based VQA. There are specific text detection based datasets about everyday generic scenes like ICDAR 2015, COCO Text, IIIT-5k. Though these datasets require the system to comprehend the text in the image, they are not specifically meant for visual question generation and visual question answering. Works such as DVQA are inclined towards question answering about graphs and plots. To read specific chart content OCR module is used. Textbook QA (TQA) considers the task of answering questions from middle-school textbooks, which basically require reasoning and understanding about text and diagrams. Reasoning about the time and date at which a photo was taken is introduced in MemexQA which also needs part of metadata for answering.
%\newline
%TextVQA proposes a new dataset which requires reading and reasoning about the scene text. It also introduces novel architecture which combines standard VQA model and an independently trained OCR module. ST-VQA is another such work which introduces source images from a number of different origins, whilst in case of TextVQA all images come from a single source, the Open Image dataset. In ST-VQA the workers who generated the question were encouraged to generate questions which can be answered unambiguously. 
 \subsection{Proposed Model}
With the presence of three modalities (answers, OCR tokens, visual features), appropriate method of combining and exploiting the features becomes important aspect of question generation. Let \textit{q} denote the question we want to generate for an image \textit{i}. This question should be generated using OCR Token \textit{tok} which is considered to be answer to the question. In this section, we explain the detailed design of the visual question generation which leverages textual content in the image. For example \ref{fig:train} if we want to generate a question for which the OCR token is \textbf{\textit{YOURNAMEHERE}} then, should consider text present in the scene i.e "YOURNAMEHERE" as an answer to generate the question. Our final goal is to define a model which should generate a question based on the OCR Token which acts as an answer. 

%TextVQA, Scene Text Visual Question Answering (ST-VQA)~\cite{}, OCR-VQA~\cite{}, T-VQA~\cite{}, DocVQA~\cite{docVQA:2021}. %\textcolor{red}{The deep learning VQA models are monolithic and predominantly have not been able to bring in the questions which are reasonable to the textual answers present along with visual content.} %Some of the works which involved inclusion of text in visual understand are DVQA~\cite{dVQA:2018}, that uses OCR to read chart content for bar-chart understanding by training models to answer questions about graphs and plots. Similar to DVQA~\cite{dVQA:2018}, FigureQA~\cite{FigureQA:2018} has yes or no questions with images characterized by bar, line and pie charts. The Textbook QA (TQA)~\cite{textbookQA:2017} answers multimodal questions from textbooks, it requires understanding and reasoning about text, diagrams and images. Though these works needs reasoning about text to answer questions, but they are confined to narrow domains like bar charts, textbook diagrams, date and time at which photo was taken (MemexQA~\cite{MemexQA:2017}), etc.
%One work that recently made a extension was DocVQA~\cite{docVQA:2021} which not only focuses on textual content but considers different document types visual cues that includes figures, forms, tables, non-textual elements and style in document images.
%The questions generated in red are not appropriate considering the scene understanding and the textual cues. Consider the first image from figure \ref{fig:res_stvqa}. The ground truth question for this image is \textit{"What six numbers are visible?"} and the generated question from the proposed method is \textit{"What is the number on the front of the train?"}. Here the OCR Token which acts as an answer to the generated question is \textbf{\textit{"222003"}}. Such successful generation of questions by our method can be attributed to its ability to semantically bridge text and objects in the image. Similarly, the example in which \textit{"calais5"} acts as the OCR Token, has generated question as \textit{"What does the sign say?"} which is almost same as that of the ground truth question which is \textit{"What is written on the sign?"}.%

